SVCCA: Singular Vector Canonical Correlation Analysis for Deep Learning Dynamics and Interpretability

We propose a new technique, Singular Vector Canonical Correlation Analysis (SVCCA), a tool for quickly comparing two representations in a way that is both invariant to affine transform (allowing comparison between different layers and networks) and fast to compute (allowing more comparisons to be calculated than with previous methods). We deploy this tool to measure the intrinsic dimensionality of layers, showing in some cases needless over-parameterization; to probe learning dynamics throughout training, finding that networks converge to final representations from the bottom up; to show where class-specific information in networks is formed; and to suggest new training regimes that simultaneously save computation and overfit less. Code: https://github.com/google/svcca/

==> Dynamics of Deep Representations (DDR)/autocrop <==
#! /bin/bash

# JBY: Autocrop.

if [ "$1" = "" ]; then
    echo "Automatically crops (a) images using convert -trim or (b) pdfs using pdfcrop."
    echo "Input filenames like filename.ext are converted to filename_crop.ext"
    echo "Files ending in _crop are skipped. Those that have already been converted to _crop"
    echo "versions are skipped based on timestamps, so it's safe to run, e.g.,"
    echo "  autocrop *pdf"
    echo "multiple times"
    echo
    echo "Usage:"
    echo " $0 file1 [ file 2 [ file 3 ... ] ]"
    exit 1
fi

while [ "$1" != "" ]; do
    filepath="$1"
    shift

    filedir=$(dirname "$filepath")
    filename=$(basename "$filepath")
    filebase="${filename%.*}"
    fileext="${filename##*.}"

    # Remove leading ./
    filedir="${filedir}/"
    if [ "$filedir" = "./" ]; then filedir=""; fi

    oldpath="${filedir}$filebase.$fileext"
    newpath="${filedir}${filebase}_crop.$fileext"

    if echo "$newpath" | grep "_crop_crop" >/dev/null; then
        echo "Skipping already cropped file $oldpath"
        continue
    fi

    if [ ! "$newpath" -nt "$oldpath" ]; then
        if [ "$fileext" = "pdf" ]; then
            pdfcrop "$oldpath" "$newpath" \
                && echo "$oldpath -> $newpath"
        else
            convert -trim +repage "$oldpath" "$newpath" \
                && echo "$oldpath -> $newpath"
        fi
    else
        echo "$oldpath -> $newpath (skipped; file already up to date)"
    fi
done


==> autocrop <==
#! /bin/bash

# JBY: Autocrop.

if [ "$1" = "" ]; then
    echo "Automatically crops (a) images using convert -trim or (b) pdfs using pdfcrop."
    echo "Input filenames like filename.ext are converted to filename_crop.ext"
    echo "Files ending in _crop are skipped. Those that have already been converted to _crop"
    echo "versions are skipped based on timestamps, so it's safe to run, e.g.,"
    echo "  autocrop *pdf"
    echo "multiple times"
    echo
    echo "Usage:"
    echo " $0 file1 [ file 2 [ file 3 ... ] ]"
    exit 1
fi

while [ "$1" != "" ]; do
    filepath="$1"
    shift

    filedir=$(dirname "$filepath")
    filename=$(basename "$filepath")
    filebase="${filename%.*}"
    fileext="${filename##*.}"

    # Remove leading ./
    filedir="${filedir}/"
    if [ "$filedir" = "./" ]; then filedir=""; fi

    oldpath="${filedir}$filebase.$fileext"
    newpath="${filedir}${filebase}_crop.$fileext"

    if echo "$newpath" | grep "_crop_crop" >/dev/null; then
        echo "Skipping already cropped file $oldpath"
        continue
    fi

    if [ ! "$newpath" -nt "$oldpath" ]; then
        if [ "$fileext" = "pdf" ]; then
            pdfcrop "$oldpath" "$newpath" \
                && echo "$oldpath -> $newpath"
        else
            convert -trim +repage "$oldpath" "$newpath" \
                && echo "$oldpath -> $newpath"
        fi
    else
        echo "$oldpath -> $newpath (skipped; file already up to date)"
    fi
done

